Galactic Token Sliding

Given a graph $G$ and two independent sets $I_s$ and $I_t$ of size $k$, the independent set reconfiguration problem asks whether there exists a sequence of $k$-sized independent sets $I_s = I_0, I_1, I_2, \ldots, I_\ell = I_t$ such that each independent set is obtained from the previous one using a so-called reconfiguration step. Viewing each independent set as a collection of $k$ tokens placed on the vertices of a graph $G$, the two most studied reconfiguration steps are token jumping and token sliding. In the token jumping variant of the problem, a single step allows a token to jump from one vertex to any other vertex in the graph. In the token sliding variant, a token is only allowed to slide from a vertex to one of its neighbors. Like the independent set problem, both of the aforementioned problems are known to be W[1]-hard on general graphs. A very fruitful line of research has showed that the independent set problem becomes fixed-parameter tractable when restricted to sparse graph classes, such as planar, bounded treewidth, nowhere-dense, and all the way to biclique-free graphs. Over a series of papers, the same was shown to hold for the token jumping problem. As for the token sliding problem, which is mentioned in most of these papers, almost nothing is known beyond the fact that the problem is polynomial-time solvable on trees and interval graphs. We remedy this situation by introducing a new model for the reconfiguration of independent sets, which we call galactic reconfiguration. Using this new model, we show that (standard) token sliding is fixed-parameter tractable on graphs of bounded degree, planar graphs, and chordal graphs of bounded clique number. We believe that the galactic reconfiguration model is of independent interest and could potentially help in resolving the remaining open questions concerning the (parameterized) complexity of token sliding.

==> Short/galactic_short.tex <==
\section{Galactic graphs and galactic token sliding}\label{sec-galactic}

We say that a graph $G = (V, E)$ is a \emph{galactic graph} when $V(G)$ is partitioned into two sets $A(G)$ and $B(G)$ where the set $A(G) \subseteq V(G)$ is the set of vertices that we call \emph{planets} and the set $B(G) \subseteq V(G)$ is the set of vertices that we call \emph{black holes}.
For a given graph $G'$, we write $G' \prec G$ whenever $|A(G')| < |A(G)|$ or, in case of equality, $|B(G')| \leq |B(G)|$.
In the standard {\sc Token Sliding} problem, tokens are restricted to sliding along edges of a graph as long as the resulting sets remain independent.
This implies that no vertex can hold more than one token and no two tokens can ever become adjacent.
In a galactic graph, the rules of the game are slightly modified. When a token reaches a black hole (a special kind of vertex), the token is
\emph{absorbed} by the black hole. This implies that a black hole can hold more than one token, in fact it can hold all $k$ tokens.
Moreover, we allow tokens to be adjacent as long as one of the two vertices is a black hole (since black holes are assumed to make tokens ``disappear''). 
On the other hand, a black hole can also ``project'' any of the tokens it previously absorbed onto any vertex in its neighborhood (be it a planet or a black hole).
Of course, all such moves require that we remain an independent set in the galactic sense.  
We say that a set $I$ is a \emph{galactic independent set} of a galactic graph $G$ whenever $G[I \cap A]$ is edgless. To fully specify a galactic independent
set $I$ of size $k$ containing more than one token on black holes, we use a weight function $\omega_I: V(G) \rightarrow \{0, \ldots, k\}$. 
Hence, $\omega_I(v) \leq 1$ whenever $v \in A(G)$, $\omega_I(v) \in \{0, \ldots, k\}$ whenever $v \in B(G)$,
and $\sum_{v \in V(G)}{\omega_I(v)} = k$.

We are now ready to define the {\sc Galactic Token Sliding} problem. We are given a galactic graph $G$, an integer $k$, and two galactic independent sets $I_s$ and $I_t$
such that $|I_s| = |I_t| = k \geq 2$ (when $k = 1$ the problem is trivial). 
The goal is to determine whether there exists a sequence of token slides
that will transform $I_s$ into $I_t$ such that each intermediate set remains a galactic independent set. As for the classical \textsc{Token Sliding} problem, given a galactic graph $G$ we can define a reconfiguration graph which we call the \emph{galactic reconfiguration graph} of $G$. It is the graph whose vertex set is the set of all galactic independent sets of $G$, two vertices being adjacent if their corresponding galactic independent sets differ by exactly one token slide.
We always assume the input graph $G$ to be a connected graph, since
we can deal with each component independently otherwise.
Furthermore, components without tokens can be safely deleted.
Given an instance $(G,k,I_s,I_t)$ of {\sc Galactic Token Sliding}, we say that $(G,k,I_s,I_t)$ can be \emph{reduced} if we
can find an instance $(G',k',I_s',I_t')$ which is positive (yes-instance) if and only if $(G,k,I_s,I_t)$ is positive and $G' \prec G$.

Let $G$ be a galactic graph. A \emph{planetary component} is a maximal connected component of $G[A]$. A \emph{planetary path} $P$, or \emph{$A$-path},
composed only of vertices of $A$, is called \emph{$A$-geodesic} if, for every $x,y$ in $P$, $\textsf{dist}_{G[A]}(x,y) = \textsf{dist}_P(x,y)$.
We use the term \emph{$A$-distance} to denote the length of a shortest path between vertices $u,v \in A$ such that all vertices of the path are also in $A$.
Let us state a few reduction rules that allow us to safely reduce an instance $(G,k,I_s,I_t)$ of {\sc Galactic Token Sliding} to an instance $(G',k',I_s',I_t')$. 

\begin{itemize}
\item Reduction rule R1 (adjacent black holes rule): If two black holes $u$ and $v$ are adjacent, we contract them into a single black hole $w$. If there are tokens on $u$ or $v$, the merged black hole receives the union of all such tokens. In other words, $\omega_{I_s'}(w) = \omega_{I_s}(u) + \omega_{I_s}(v)$ and $\omega_{I_t'}(w) = \omega_{I_t}(u) + \omega_{I_t}(v)$. Loops and multi-edges are ignored.
 
\item Reduction rule R2 (dominated black hole rule): If there exists two black holes $u$ and $v$ such that $N(u) \subseteq N(v)$, $\omega_{I_s}(u) = 0$, and $\omega_{I_t}(u) = 0$, we delete $u$. 

\item Reduction rule R3 (absorption rule): If there exists $u,v$ such that $u$ is a black hole, $v \in N(u) \cap A$ ($v$ is a neighboring planet that could be in $I_s \cup I_t$) and  $|((I_s \cup I_t) \cap A ) \cap N[v]| \leq 1$, then we contract the edge $uv$. We say that $v$ is \emph{absorbed} by $u$. If $v \in I_s \cup I_t$ then we update the weights of $u$ accordingly.
 
\item Reduction rule R4 (twin planets rule): Let $u,v \in A(G)$ be two planet vertices that are \emph{twins} (true or false twins). That is, either $uv \not\in E(G)$ and $N(u) = N(v)$ or $uv \in E(G)$ and $N[u] = N[v]$. 
If $u \not\in I_s \cup I_t$ then delete $u$. 
If both $u$ and $v$ are in $I_s$ (resp. $I_t$) and at least one of them is not in $I_t$ (resp. $I_s$) then return a trivial no-instance. If both $u$ and $v$ are in $I_s$ as well as $I_t$ then delete $N[u] \cup N[v]$, decrease $k$ by two, and set $I_s' = I_s \setminus \{u,v\}$ and $I_t' = I_t \setminus \{u,v\}$. 

\item Reduction rule R5 (path reduction rule): Let $G$ be a galactic graph and $P$ be a $A$-geodesic path of length at least $5k$ such that  $(A \cap N[P]) \cap (I_s \cup I_t) = \emptyset$. Then, $P$ can be contracted into a black hole (we ignore loops and multi-edges). That is, we contract all edges in $P$ until one vertex remains. 
\end{itemize}

As immediate consequences, the following properties hold in an instance where reduction rules R1 to R5 cannot be applied.

\begin{corollary}\label{cor:planet-neighbor}
Each (planet) neighbor of a black hole must have at least two vertices of $I_s \cup I_t$ in its planet neighborhood.
\end{corollary}

\begin{corollary}\label{cor-planet-components}
Every planetary component must contain at least one token and therefore $G$ can have at most $k$ planetary components, when $k \geq 2$.
\end{corollary}

\begin{corollary}\label{cor-diam}
Let $(G,k,I_s,I_t)$ be an instance of {\sc Galactic Token Sliding} where reduction rules R1, R3, and R5 (adjacent black holes rule, absorption rule, and the path reduction rule) have been exhaustively applied. Then, the graph $G$ has diameter at most $O(k^2)$. Moreover, any planetary component has diameter at most $O(k^2)$.
\end{corollary}

We now show how the galactic reconfiguration framework combined with the previous reduction rules immediately implies that \textsc{Token Sliding} is fixed-parameter tractable for parameter $k + \Delta(G)$, where $\Delta(G)$ denotes the maximum degree of $G$. Theorem~\ref{thm:ts-bounded-degree-fpt} immediately implies  positive results for graphs of bounded bandwidth/bucketwidth. 

\begin{theorem}\label{thm:ts-bounded-degree-fpt}
\textsc{Token Sliding} is fixed-parameter tractable when parameterized by $k + \Delta(G)$. Moreover, the problem admits a bikernel\footnote{A kernel where the resulting instance is not an instance of the same problem.} with $k\Delta(G)^{O(k^2)} + (2k + 2k\Delta(G))\Delta(G)$ vertices. 
\end{theorem}

\begin{proof}
Let $(G, k, I_s, I_t)$ be an instance of \textsc{Token Sliding}. We first transform it to an instance of \textsc{Galactic Token Sliding} where all vertices are planetary vertices. We then apply all of the reduction rules R1 to R5 exhaustively. By a slight abuse of notation we let $(G, k, I_s, I_t)$ denote the irreducible instance of \textsc{Galactic Token Sliding}.

The total number of planetary components in $G$ is at most $k$ by Corollary~\ref{cor-planet-components} and the diameter of each such component is at most $O(k^2)$ by Corollary~\ref{cor-diam}. Hence the total number of planet vertices is at most $k\Delta(G)^{O(k^2)}$. 

To bound the total number of black holes, it suffices to note that no black hole can have a neighbor in $B \cup (A \setminus N[I_s \cup I_t])$. In other words, no black hole can be adjacent to another black hole (since the adjacent black holes reduction rule would apply) and no black hole can be adjacent to a planet without neighboring tokens (otherwise the absorption reduction rule would apply). Hence, combined with the fact that each black hole must have degree at least one, the total number of black holes is at most $(2k + 2k\Delta(G))\Delta(G)$.
\end{proof}

%Theorem~\ref{thm:ts-bounded-degree-fpt} immediately implies  positive results for graphs of bounded bandwidth/bucketwidth. 
%The bandwidth of a graph is the minimum over all assignments $f: V(G) \rightarrow \mathbb{N}$ of the quantity $\mathrm{max}_{uv \in E(G)} |f(u) - f(v)|$. A graph of bandwidth $b$ can easily
%be seen to have pathwidth and treewidth at most $b$ and maximum degree at most $2b$. On the other hand, the family of stars $K_{1,n}$ gives an example with bounded pathwidth but unbounded bandwidth. A bucket arrangement of a graph is a partition of the vertex set into a sequence of buckets, such that the endpoints of any edge are either in one bucket or in two consecutive buckets. If a graph has a bucket arrangement where each bucket has at most $b$ vertices, then it has bandwidth at most $2b$ (arrange one bucket after another, with any ordering within one bucket).


==> Short/intro_short.tex <==

\section{Introduction}\label{sec-intro}

Many algorithmic questions can be represented as follows:
given the description of a system state and the description of a state we would ``prefer'' the system to be in, is it possible to transform the system
from its current state into the more desired one without ``breaking'' the system in the process? And if yes, how many steps are needed? Such problems naturally arise in the fields of mathematical puzzles, operational research, computational geometry~\cite{DBLP:journals/comgeo/LubiwP15}, bioinformatics,  and quantum computing~\cite{DBLP:conf/icalp/GharibianS15} for instance. These questions received a substantial amount of attention under the so-called \emph{combinatorial reconfiguration framework} in the last few years~\cite{DBLP:journals/tcs/BrewsterMMN16,H13,Wrochna15}.
We refer the reader to the surveys by van den Heuvel~\cite{H13}
and Nishimura~\cite{DBLP:journals/algorithms/Nishimura18} for more background on combinatorial reconfiguration.

\subparagraph*{Independent set reconfiguration.} In this work, we focus on the reconfiguration of independent sets.
Given a simple undirected graph $G$, a set of vertices $S \subseteq V(G)$ is an \emph{independent set} if the vertices
of $S$ are all pairwise non-adjacent. Finding an independent set of maximum cardinality, i.e., the {\sc Independent Set} problem,
is a fundamental problem in algorithmic graph theory and is known to be not only \NPP-hard, but also \WO-hard and
not approximable within $\Oh(n^{1-\epsilon})$, for any $\epsilon > 0$, unless $\PP = \NPP$~\cite{DBLP:journals/toc/Zuckerman07}.
Moreover, {\sc Independent Set} is known to remain \WO-hard on graphs excluding $C_4$ (the cycle on four vertices) as an induced subgraph~\cite{DBLP:conf/iwpec/BonnetBCTW18}.

We view an independent set as a collection of tokens placed on the vertices of a graph such that no two tokens are adjacent.
This gives rise to two natural adjacency relations between independent sets (or token configurations), also called \emph{reconfiguration steps}.
These two reconfiguration steps, in turn, give rise to two combinatorial reconfiguration problems.
In the {\sc Token Jumping} (TJ) problem, introduced by Kami\'{n}ski et al.~\cite{KMM12}, a single reconfiguration step consists of first removing a token on some vertex $u$ and then immediately adding it back on any other vertex $v$, as long as no two tokens become adjacent. The token is said to \emph{jump} from vertex $u$ to vertex $v$.
In the {\sc Token Sliding} (TS) problem, introduced by Hearn and Demaine~\cite{DBLP:journals/tcs/HearnD05}, two independent sets are adjacent if one can be obtained from the other by a token jump from vertex $u$ to vertex $v$ with the additional requirement of $uv$ being an edge of the graph. The token is then said to \emph{slide} from vertex $u$ to vertex $v$ along the edge $uv$. Note that, in both the TJ and TS problems, the size of independent sets is fixed.
Generally speaking, in the {\sc Token Jumping} and {\sc Token Sliding} problems,
we are given a graph $G$ and two independent sets $I_s$ and $I_t$ of $G$. The goal is to determine
whether there exists a sequence of reconfiguration steps -- a \emph{reconfiguration sequence} -- that
transforms $I_s$ into $I_t$ (where the reconfiguration step depends on the problem).

Both problems have been extensively studied, albeit under
different names~\cite{DBLP:conf/wg/BonamyB17,DBLP:conf/swat/BonsmaKW14,demaine_linear-time_2015,DBLP:conf/isaac/Fox-EpsteinHOU15,DBLP:conf/tamc/ItoKOSUY14,DBLP:journals/ieicet/ItoNZ16,KMM12,lokshtanov_reconfiguration_2018}.
It is known that both problems are \PPSPACE-complete, even on restricted graph classes such as
graphs of bounded bandwidth (and hence pathwidth)~\cite{WROCHNA14} and planar graphs~\cite{DBLP:journals/tcs/HearnD05}. 
%
On the positive side, it is easy to prove that {\sc Token Jumping} can be decided in polynomial time on trees (and even on chordal graphs) since we simply have to iteratively jump tokens to leaves (resp. vertices that only appear in the bag of a leaf in the clique tree) to transform an independent set into another. Unfortunately, for {\sc Token Sliding}, the problem becomes more complicated because of what we call the \emph{bottleneck effect}. Indeed, there might be a lot of empty leaves in the tree but there might be a bottleneck in the graph that prevents us from reaching these desirable vertices. For instance, consider a star plus a long subdivided path attached to the center of the star. One cannot move any token from the  leaves of the star to the path if there are at least two tokens on the leaves (in other words, two tokens adjacent to a cut-vertex prevent us from using the cut vertex). 
Even if we can overcome this issue for instance on trees~\cite{demaine_linear-time_2015} and on interval graphs~\cite{DBLP:conf/wg/BonamyB17}, the {\sc Token Sliding} problem remains much ``harder'' than the {\sc Token Jumping} problem. In split graphs for instance (which are chordal), {\sc Token Sliding} is PSPACE-complete~\cite{DBLP:conf/stacs/Belmonte0LMOS19}. Lokshtanov and Mouawad~\cite{DBLP:journals/talg/LokshtanovM19} showed that, in bipartite graphs, {\sc Token Jumping} is \NPP-complete
while {\sc Token Sliding} remains \PPSPACE-complete. 

In this paper we focus on the parameterized complexity of the {\sc Token Sliding} problem. While the complexity of {\sc Token Jumping} parameterized by the size of the independent set is quite well understood, the comprehension of the complexity of {\sc Token Sliding} remains evasive.
%
A problem $\Pi$ is \FPT\ (fixed-parameterized tractable) parameterized by $k$ if one can solve it in time $f(k) \cdot poly(n)$, for some computable function $f$. In other words, the combinatorial
explosion can be restricted to a parameter $k$. In the rest of the paper, our parameter $k$ will be the size of the independent set (i.e.\ number of tokens).
Both {\sc Token Jumping} and {\sc Token Sliding} are known to be \WO-hard\footnote{Informally, it means that they are very unlikely to admit an \FPT\ algorithm.}
parameterized by $k$ on general graphs~\cite{lokshtanov_reconfiguration_2018}.
%
On the positive side, Lokshtanov et al.~\cite{lokshtanov_reconfiguration_2018} showed that {\sc Token Jumping} is \FPT\ on bounded degree graphs. This result has been extended in a series of papers to planar graphs, nowhere-dense graphs, and finally strongly $K_{\ell,\ell}$-free graphs~\cite{IKO14,klasing_token_2017}, a graph
being strongly $K_{\ell,\ell}$-free if it does not contain any $K_{\ell,\ell}$ as a subgraph. 
%
For {\sc Token Sliding}, it was proven in~\cite{DBLP:journals/algorithmica/BartierBDLM21} that the problem is \WO-hard on bipartite graphs and $C_4$-free graphs (a similar result holds for {\sc Token Jumping} but based on  weaker assumptions for the bipartite case~\cite{DBLP:conf/iwpec/AgrawalAD21}).

Almost no positive result is known for {\sc Token Sliding} even for incredibly simple cases like graphs of bounded degree. Our main contributions are to develop two general tools for the design of parameterized algorithms for {\sc Token Sliding}, namely galactic reconfiguration and types. Galactic reconfiguration is a general simple tool that allows us to reduce instances. Using it, we will derive that {\sc Token Sliding} is \FPT\ on bounded degree graphs.
Our second tool, called types, will in particular permit to show that when the deletion of a small subset of vertices leaves too many components, then one of them can be removed. 
Combining both tools with additional rules, we prove that {\sc Token Sliding} is \FPT\ on planar graphs and on chordal graphs of bounded clique number. We complement these results by proving that {\sc Token Sliding} is \WO-hard on split graphs.

\subparagraph{Galactic reconfiguration.} 
%Our goal in this paper is to give the basis of the study of {\sc Token Sliding}. 
Our first result is the following:

\begin{theorem}\label{thm:ts-bounded-degree-fpt-intro}
{\sc Token Sliding} is \FPT\ on bounded degree graphs parameterized by $k$.
\end{theorem}

Much more than the result itself, we believe that our main contribution here is the general framework we developed for its proof, namely galactic reconfiguration.
%
Before explaining exactly what it is, let us explain the intuition behind it. As we already said, even if there are vertices which are far apart from the vertices of an independent set, we are not sure we can reach them because of the bottleneck effect. Our intuition was that it should be possible to reduce a part of large diameter of the graph that does not contain any tokens (just as we can find irrelevant vertices when we have large grid minors). The idea is that since the diameter is large, we should be able to hide tokens far apart from each other in this structure, avoiding the ``bottleneck issue''. And thus the structure should be reducible.
%since when we enter in the structure, we can basically move as we want in it (and then avoid to put tokens close to each other) \textcolor{red}{why grid minor in particular?}. 
However, proving that a structure can be  reduced in reconfiguration is usually very technical. To overcome this problem, we introduce a new type of vertices called \emph{black holes} which can swallow as many tokens of the independent set as we like. 
A \emph{galactic graph} is a graph that might contain black holes. 
%A \emph{galactic independent set} is a set of tokens such that the set of tokens on non black-hole vertices is an independent set and each black hole might contain as tokens as we like.
A \emph{galactic independent set} is a set of vertices on which tokens lie, such that the set of non black hole vertices holding tokens is an independent set and such that each black hole might contain any number of tokens.

Our main result is to prove that if there exists a long shortest path that is at distance two from the initial and target independent sets, then we can replace it by a black hole (whose neighborhood is the union of the neighborhoods of the path).  This rule, together with other simple rules on galactic graphs, allows us to reduce the size of bounded-degree graphs until they reach a size of at most $f(k)$, for some computable function $f$, in polynomial time. Since a kernel ensures the existence of an \FPT\ algorithm, Theorem~\ref{thm:ts-bounded-degree-fpt-intro} holds.

\subparagraph*{Types and the multi-component reduction.}
In the rest of the paper, we combine galactic graphs with other techniques to prove that {\sc Token Sliding} is \FPT\ on several other graph classes.  We first prove the following:

\begin{theorem}\label{thm:ts-planar-intro}
{\sc Token Sliding} is \FPT\ on  planar graphs parameterized by $k$.
\end{theorem}

To prove Theorem~\ref{thm:ts-planar-intro}, we cannot simply use our previous long path construction since, in a planar graph, there might be a universal vertex which prevents the existence of a long shortest path. Note that the complexity of {\sc Token Sliding} is open on outerplanar graphs and it was not known to be \FPT\ prior to our work.

Our strategy consists in reducing to planar graphs of bounded degree and then applying Theorem~\ref{thm:ts-bounded-degree-fpt-intro}.
To do so, we provide another general tool to reduce graphs for {\sc Token Sliding}. Namely, we show that if there is a set $X$ of vertices such that $G - X$ contains too many connected components (in terms of $k$ and $|X|$) then at least one of them can be safely removed. 
%
The idea of the proof consists in defining the \emph{type} of a connected component of $G-X$. From a very high level perspective, the type\footnote{The exact definition is actually more complicated.} of a path in a component of $G - X$ is the sequence of its neighborhoods in $X$. The type of a component $C$ is the union of the types of the paths starting on a vertex of $C$. We then show that if too many components of $G-X$ have the same type then one of them can be removed.
%

However, this component reduction is not enough since, in the case of a vertex universal $x$ to an outerplanar graph, the deletion of $x$ does not leave many connected components. We prove that, we can also reduce a planar graph if (i) there are too many vertex-disjoint $(x,y)$-paths for some pair $x,y$ of vertices or, (ii) if a vertex has too many neighbors on an induced path. Since one can prove that in an arbitrarily large planar graph with no long shortest path (i) or (ii) holds, it will imply Theorem~\ref{thm:ts-planar-intro}.

Note that our proof techniques can be easily adapted to prove that the problem is \FPT\ for any graph of bounded genus. 
We think that the notion of types may be crucial to derive \FPT\ algorithms on larger classes of graphs such as bounded treewidth graphs.

We finally provide another application of our method by proving that the following holds:

\begin{theorem}\label{thm:ts-chordal-bounded-clique-intro}
{\sc Token Sliding} is \FPT\ on chordal graphs of bounded clique number.
\end{theorem}

The proof of Theorem~\ref{thm:ts-chordal-bounded-clique-intro} consists in proving that, since there is a long path in the clique tree, we can either find a long shortest path (and we can reduce the graph using galactic graphs) or find a vertex $x$ in a large fraction of the bags of this path. In the second case, we show that we can again reduce the graph.
We complement this result by proving that it cannot be extended to split graphs, contrarily to {\sc Token Jumping}.

\begin{theorem}
{\sc Token Sliding} is \WO-hard on split graphs.
\end{theorem}

We show hardness via a reduction from the \textsc{Multicolored Independent Set} problem, known to be \WO-hard~\cite{DBLP:books/sp/CyganFKLMPPS15}. The crux of the reduction relies on the fact that we have a clique of unbounded size and hence we can use different subsets of the clique to encode vertex selection gadgets and non-edge selection gadgets.

\subparagraph*{Further work.}
The first natural generalization of our result on chordal graphs of bounded clique size would be the following:

\begin{question}\label{q:treewidth}
Is {\sc Token Sliding} \FPT\ on bounded treewidth graphs? Or simpler, on bounded pathwidth graphs?
\end{question}

Recall that the problem is \PPSPACE-complete on graphs of constant bandwidth for a large enough constant that is not explicit in the proof~\cite{WROCHNA14}. 
Note that our galactic reconfiguration rules directly ensure that {\sc Token Sliding} is \FPT\ on bounded bandwidth graphs and the multi-component reduction ensures that the problem is \FPT\ for graphs of bounded treedepth. But even for bounded pathwidth, the situation is unclear. There are good indications to think that solving the bounded pathwidth case is the hardest step to obtain an \FPT\ algorithm for bounded treewidth graphs.
%
On the positive side, we simply know that the problem is polynomial time solvable on graphs of treewidth one (namely forests)~\cite{demaine_linear-time_2015} and the problem is open for outerplanar graphs, which are graphs of treewidth $2$:

\begin{question}
Is {\sc Token Sliding} polynomial-time solvable on outerplanar graphs? Triangulated outerplanar graphs?
\end{question}

We did not succeed in answering Question~\ref{q:treewidth} but we think that the method we used for Theorem~\ref{thm:ts-chordal-bounded-clique-intro} is a good starting point (with a much more involved analysis).
%
In the case of {\sc Token Jumping} the problem is actually \FPT\ on strongly $K_{\ell,\ell}$-free graphs which contains planar graphs, bounded treewidth graphs, and many other classes. If the answer to Question~\ref{q:treewidth} is positive, the next step to achieve a similar statement for {\sc Token Sliding} would consist in looking at minor-free graphs and, more generally, nowhere dense graphs.

\subparagraph*{Organization of the paper.} In Section~\ref{sec-galactic}, we formally introduce galactic graphs and provide our main reduction rules concerning such graphs, including the long shortest path reduction lemma. In Section~\ref{sec-components}, we introduce the notion of types and journeys and prove that if there are too many connected components in $G - X$ then at least one of them can be removed. In Section~\ref{sec-planar}, we prove that {\sc Token Sliding} is \FPT\ on planar graphs. We prove the same for chordal graphs of bounded clique number, and finally give our hardness reduction for split graphs in the appendix. Omitted proofs can be found in the full version of the paper attached in the appendix. 

==> Short/multicomponent_short.tex <==
\section{The multi-component reduction rule  (R6)}\label{sec-components}

\subparagraph*{General idea.}
The goal of this section is to show how we can reduce a graph when we have a small vertex separator with many components attached to it. We let $X$ be a subset of vertices and $H$ be an induced subgraph of $G - X$ (for simplicity we assume $G$ is a non-galactic graph in this section). Let $I_{s}$ and $I_{t}$ be two independent sets which are disjoint from $H$ and consider a reconfiguration sequence from $I_s$ to $I_t$ in $G$. Let $v$ be a vertex of $H$ and assume that there is a token $t$ that is \emph{projected} on $v$ at some point of the reconfiguration sequence, meaning that the token $t$ is moved from a vertex of $X$ to $v$.
This token may stay a few steps on $v$, move to some other vertex $w$ of $H$, and so on until it eventually goes back to $X$. Let this sequence of vertices (allowing duplicate consecutive vertices) be denoted by $v_1=v,v_2,\ldots,v_r$. We call this sequence the \emph{journey} of $v$ (formal definitions are given in the next subsection). 

Assume now that the number of connected components attached to $X$ is arbitrarily large. Our goal is to show that one of those components can be safely deleted, that is, without compromising the existence of a reconfiguration sequence if one exists.
Suppose that we decide to delete the component $H$.
The transformation from $I_s$ to $I_t$ does not exist anymore since, in the reconfiguration sequence, the token $t$ was projected on $v \in V(H)$.
But we can ask the following question:
Is it possible to simulate the journey of $v$ in another connected component of $G - X$? 
In fact, if we are able to find a vertex $w$ in a connected component $H' \neq H$ of $G - X$ and a sequence $w_1=w,\ldots,w_r$ of vertices such that $w_iw_{i+1}$ is an edge for every $i$ and such that $N(w_i) \cap X = N(v_i) \cap X$, then we could project the token $t$ on $w$ instead of $v$ and perform this journey instead of the original journey\footnote{We assume for simplicity in this outline that the component of $w$ does not contain tokens.} of $t$.
One possible issue is that the number $r$ of (distinct) vertices in the journey can be arbitrarily large, and thus the existence of $w$ and $H'$ is not guaranteed \textit{a priori}. 
This raises more questions:
What is really important in the sequence $v=v_1,v_2,\ldots,v_r$?
Why do we go from $v_1$ to $v_r$?
Why so many steps in the journey if $r$ is large?
The answers, however, are not necessarily unique.
We distinguish two cases.

First, suppose that in the reconfiguration sequence, the token $t$ was projected from $X$ to $v$, performed the journey without having to ``wait'' at any step (so no duplicate consecutive vertices in the journey), and then was moved to a vertex $x' \in X$. Then, the journey only needs to ``avoid'' the neighbors of the vertices in $X$ that contain a token.
Let us denote by $s_1$ the step where the token $t$ is projected on $v$ and by $s_2$ the last step of the journey (that is, the step where $t$ is one move/slide away from $X$).
Let $Y$ be the vertices of $X$ that contain a token between the steps $s_1$ and $s_2$. 
The journey of $t$ can then be summarized as follows: a vertex whose neighborhood in $X$ is equal to $N(v) \cap X$, a walk whose vertices all belong to $H$ and are only adjacent to subsets of $X \setminus Y$, and then a vertex whose neighborhood in $X$ is equal to $N(v_r) \cap X$. 
In particular, if we can find, in another connected component of $G-X$, a vertex $w$ for which such a journey (with respect to the neighborhood in $X$) also exists, then the we can project $t$ on $w$ instead of $v$.
Clearly, the obtained reconfiguration sequence would also be feasible (assuming again no other tokens in the component of $w$).

However, we might not be able to go ``directly'' from $v_1=v$ to $v_r$. Indeed, at some point in the sequence, there might be a vertex $v_{i_1}$ which is adjacent to a token in $X$.
This token will eventually move (since the initial journey  with $t$ in $H$ is valid), which will then allow the token $t$ to go further on the journey.
But then again, either we can reach the final vertex $v_r$ or the token $t$ will have to wait on another vertex $v_{i_2}$ for some token on $X$ to move, and so on (until the end of the journey). We say that there are \emph{conflicts} during the journey\footnote{Actually, there might exist another type of conflict we do not explain in this outline for simplicity.}.

So we can now "compress" the path as a path from $v_1$ to $v_{i_1}$, then from $v_{i_1}$ to $v_{i_2}$ (together with the neighborhood in $X$ of these paths), as we explained above.
However, we cannot yet claim that we have reduced the instance sufficiently since the number of conflicts is not known to be bounded (by a function of $k$ and/or the size of $X$). The main result of this section consists in proving that, if we consider a transformation from $I_{s}$ to $I_{t}$ that minimizes the number of moves ``related'' to $X$, then (almost) all the journeys have a ``controllable'' amount of (so-called important) conflicts. Actually, we prove that, in most of the connected components $H$ of $G - X$, we can assume that we have a "controllable" number of important conflicts for every journey on $H$ in a transformation that minimizes the number of token modifications involving $X$. The idea consists in proving that, if there are too many important conflicts during a journey of a token $t$, we could mimic the journey of $t$ on another component to reduce the number of token slides involving $X$.

Finally, we will only have to prove that if all the vertices have a controllable number of conflicts (and there are too many components), then we can safely delete a connected component of $G - X$.

\subparagraph*{Journeys and conflicts.}
We denote a reconfiguration sequence from $I_s$ to $I_t$ by $\mathcal{R} = \langle I_0,I_1,\ldots,I_{\ell-1},I_\ell \rangle$. 
Let $X \subseteq V(G)$ and $H$ be a component in $G - X$ such that $I_s \cap V(H) = I_t \cap V(H) = \emptyset$. All along this section, we are assuming that tokens have labels just so we can keep track of them. For every token $t$, let $v_i(t)$, $0 \leq i \leq \ell$, denote the vertex on which token $t$ is at position $i$ in the reconfiguration sequence $\mathcal{R}$.

Whenever a token enters $H$ and leaves it, we say that the token makes a journey in $H$.  Let $I_i$ denote the first independent set in $\mathcal{R}$ where $v_i(t) \in V(H)$ and let $I_j$, $i \le j$, denote the first independent set after $I_i$ where $v_{j+1}(t) \not\in V(H)$. Then the \emph{journey $J$ of $t$ in $H$} is the sequence $(v_i(t), \ldots, v_j(t))$. The journey is a sequence of vertices (with multiplicity) from $H$ such that consecutive vertices are either the same or connected by an edge. We associate each journey $J$ with a walk $W$ in $H$. The \emph{walk $W$ of $t$} in $H$ is the journey of $t$ where duplicate consecutive vertices have been removed.

We say that a token is \emph{waiting at step $i$} if $v_i(t) = v_{i-1}(t)$; otherwise the token is \emph{active}. 
Given a journey $J$ and its associated walk $W$, we say that $w \in W$ is a \emph{waiting vertex} if there is a step where the vertex $w$ is a waiting vertex in the journey.
%Those vertices (that differentiate the journey from the walk) are what we call \emph{waiting vertices}. 
Otherwise $w$ is an \emph{active vertex} (with respect to the reconfiguration sequence). 
So we can now decompose the walk $W$ into waiting vertices and transition walks. That is, assuming the walk starts at $y$ and ends at $z$, we can write $W = y P_0 w_0 P_1 w_1 \ldots w_\ell P_\ell z$, where each $w_i$ is a waiting vertex and each $P_i$ is a \emph{transition walk} (consisting of the walk of active vertices between two consecutive waiting vertices). Note that the transition walks could be empty. 

We are interested in why a token $t$ might be waiting at some vertex $w$. In fact, we will only care about waiting vertices that we will call important waiting vertices.
Let $w_1,\ldots,w_\ell$ be the waiting vertices of the journey and, for every $i \le \ell$, let us denote by $[s_i,s'_i]$ the time interval of the reconfiguration sequence where the token $t$ is staying on the vertex $w_i$. Note that $s_i < s_i'$. Also note that when $t$ is active the other tokens are not moving; thus the position of any token different from $t$ is the same all along the interval $[s_i'+1,s_{i+1}]$ for every $i \le \ell-1$.

Let $i < j \le \ell$ and let $w_i$ be a waiting vertex. 
We say that $w_j$ is the \emph{important waiting vertex after $w_i$} if $j>i$ and $j$ is the largest integer such that no vertex along the walk of token $t$ between $w_i$ (included) and $w_j$ (included) is adjacent to a token $t' \neq t$ or contains a token $t' \neq t$ between steps $s_i'$ and $s_j$ (note that the important waiting vertex after $w_i$ might be the last vertex of the sequence). Since token $t$ is active from $s_i' + 1$ to $s_{i+1}$ and is moving from $w_i$ to $w_{i+1}$ during that interval, the important waiting vertex after $w_i$ is well-defined and is at least $w_{i+1}$. Let $Q_{i,j}$ denote the walk in $H$  that the token $t$ follows to go from $w_i$ to $w_j$ (both $w_i$ and $w_j$ are included in $Q_{i,j}$). In other words, $Q_{i,j}=w_iP_{i+1}w_{i+1}\ldots P_jw_j$.
Now, note that since $w_j$ is the important waiting vertex after $w_i$ (i.e. we cannot replace $w_j$ by $w_{j+1}$), then we claim that the following holds:

\begin{claim}\label{clm:defconflict}
If $w_j$ is not the last vertex of the walk $W$, either 
\begin{enumerate}[(i)]
    \item\label{c1} there is a token on or adjacent to a vertex of $P_{j+1}w_{j+1}$ (the transition walk after $w_j$) at some step in $[s_i',s_j']$ or,
    \item\label{c2} there is a token on or adjacent to a vertex of $Q_{i,j} - w_j$ in the interval $[s_j,s_{j+1}]$.
\end{enumerate}
\end{claim}

Let us now define the notion of conflicts. Since we cannot replace $w_j$ by $w_{j+1}$, it means that, by definition, there is at least one step $s_q$ in $[s_i',s_{j+1}]$ where a token $t_q \ne t$ is adjacent to (or on a vertex) $v_q$ of $Q_{i,j+1}$. We call such a step a \emph{conflict}. We say that $(s_q,v_q,t_q)$ is the \emph{conflict triplet} associated to the conflict (for simplicity, we will mostly refer to a triplet as a conflict). 

%We can now prove Claim~\ref{clm:defconflict}.
%\begin{proof}
%If the token is (on or) adjacent to $Q_{i,j}$, it cannot be in the interval $[s_i',s_j]$ by definition of $w_j$. So, if we are in case (ii), the conflict with $t'$ is after step $s_j$. And since $t$ is waiting on $w_j$, the conflict is indeed with a vertex in $V(Q_{i,j}) \setminus w_j$.
%If we are in the case (i), the conflict can hold at any step between $s_i'$ and $s_j$. Note however that, after step $s_j'$, the token $t$ becomes active and goes from $w_j$ to $w_{j+1}$ in the sequence. So there is no token anymore in the neighborhood of $P_{j+1}w_{j+1}$ at step $s_j'$. In other words, if we have conflicts of type (i), there is a last such conflict in the interval $[s_i',s_j']$. 
%And if we have conflicts of type (ii), there is a first conflict in the interval $[s_j,s_j']$.
%\end{proof}

The conflicts of type (i) are called \emph{right conflicts} and the conflicts of type (ii) are called  \emph{left conflicts}. It might be possible that $w_j$ is the important waiting vertex because we have (several) left and right conflicts. We say that $w_j$ is a \emph{left important vertex} if there is at least one left conflict and a \emph{right important vertex} otherwise.
 
If $w_j$ is a left important vertex, we let the \emph{important conflict} $(s_\star,v_\star,t_\star)$ denote the first conflict associated with $Q_{i,j}$ between steps $s_j$ and $s_j'$, i.e., there exists no $s$ such that $s_j \leq s < s_\star  \leq s_j'$ such that there is a conflict at step $s$ with a token $t' \ne t$ which is either on $Q_{i,j}$ or incident to $Q_{i,j}$. 
Note that $v_\star$ cannot be a vertex of $Q_{i,j}$ since that would imply at least one more conflict before $s_\star$, hence $v_\star \in N(V(Q_{i,j}))$. 

If $w_j$ is a right important vertex, we let $(s_\star,v_\star,t_\star)$ denote the \emph{important conflict} associated with $P_{j+1}w_{j+1}$ between steps $s_i'$ and $s_j'$ as the last conflict associated to $P_{j+1}w_{j+1}$, i.e., there exists no $s$ such that $s_i' \leq s_\star < s \leq s_j'$ and there is a conflict $(s,v_s,t_s)$ such that $v_s$ in $P_{j+1}w_{j+1}$ or incident to $P_{j+1}w_{j+1}$. Note that $v_\star$ cannot be a vertex of $P_{j+1}w_{j+1}$ since that would imply at least one more conflict after $s_\star$, hence $v_\star \in N(V(P_{j+1}w_{j+1}))$. 
We use $\mathcal{C}(Q_{i,j + 1})[s_i', s_j']$ to denote all conflict triplets (left and right conflicts) associated with $Q_{i,j + 1}$ between steps $s_i'$ and $s_j'$.

To conclude this section, let us remark that the conflicts might be due to vertices of $H$ or vertices of $X$. In other words, for a conflict triple $(s, v, t) \in \mathcal{C}(Q_{i,j + 1})[s_i', s_j']$, $v$ is an $H$-conflict or an $X$-conflicts depending on whether $v$ is in $X$ or in $H$. In what follows we will only be interested in $X$-conflicts. The \emph{$X$-important waiting vertex after $w_i$} is $w_j$ where $j > i$ is the smallest integer such that 
$\mathcal{C}(Q_{i,j + 1})[s_i', s_j']$ contains at least one triplet 
$(s, v, t')$ where $t' \neq t$, $v \in X$, and $s_i' \leq s \leq s_j'$. Now given a journey we can define the sequence of $X$-important waiting vertices as the sequence $w'_1,\ldots,w'_r$ starting with vertex $w_1$ and such that $w'_{j+1}$ is the $X$-important waiting vertex after $w_j$. What will be important in the rest of the section is the length $r$ of this sequence. If this sequence is short (bounded by $f(k)$), then we can check if we can simulate a similar journey in other components efficiently. If the sequence is long, we will see that it implies that we can find a "better" transformation.

Since we will mostly be interested in how a journey interacts with $X$, we introduce the notion of the $X$-walk associated with journey $J$. The \emph{$X$-walk} is  written as $W^X = y P_0 w_0 P_1 w_1 \ldots w_\ell P_\ell z$, where each $w$ is an $X$-important waiting vertex and each $P$ is the walk that the token takes (note that this walk could have non-important waiting vertices) before reaching the next $X$-important waiting vertex. We call each $P$ in an $X$-walk an \emph{$X$-transition walk}. 

\subparagraph*{Types and signatures.}
Let $X$ be a subset of vertices and $H$ be a component of $G - X$. An \emph{$\ell$-type} is defined as a sequence 
$I Y_1 W_1 Y_2 W_2 \ldots Y_\ell W_\ell Y_{\ell + 1} F$ such that for every $i$, $W_i$ is a (possibly empty) subset of $X$ and $Y_i$ is a (possibly empty) subset of $X$ or a special value $\perp$ (the meaning of $\perp$ will become clear later on). We call $I$ the \emph{initial value} and $F$ the \emph{final value} and they are both non-empty subsets of vertices of $X$. 
The $0$-type is defined as $I Y_0 F$ and we allow $I$ to be equal to $F$. 
%\commentN{What is a $0$-type. i.e. what do we do if we have no waiting vertex? Should we say that it is $I Y_0 F$ ? If $Y_0 = \perp$ are we assuming that $I$ might be equal to $F$?}
%\commentA{Yes the 0-type should be IYF if I and F are different and just I otherwise no? This should not matter for rest of the exposition though.}
We will often represent an $\ell$-type by $(I (Y_iW_i)_{i \le \ell}Y_{\ell + 1} F)$. Note that if $X$ is bounded, then the number of $\ell$-types is bounded. More precisely, we have:

\begin{remark}\label{rem:nr-types}
The number of $\ell$-types is at most $(2^{|X|}+1)^{2(\ell+2)}$.
\end{remark}

The neighborhood of a set of vertices $S \subseteq V(H)$ in $X$ is called the \emph{$X$-trace} of $S$. 
A journey $J$ is \emph{compatible} with an $\ell$-type $I Y_1 W_1 Y_2 W_2 \ldots Y_\ell W_\ell Y_{\ell+1} F$ if it is possible to partition the $X$-walk $W$ of $J$ into $W^X = y P_0 w_0 P_1 w_1 \ldots P_\ell w_\ell P_{\ell + 1} z$ such that:
\begin{itemize}
    \item the $X$-trace of each vertex $w_i$ is $W_i$, 
    \item for every walk $P_i$ which is not empty, the $X$-trace of $P_i$ is $Y_i$, i.e., $\cup_{x \in P_i} N(x) \cap X = Y_i$ (note that we can have $Y_i = \emptyset$), 
    \item for every empty walk $P_i$, we have $Y_i=\perp$, and
    \item the $X$-trace of $y$ is $I$ and the $X$-trace of $z$ is $F$. 
\end{itemize}
%
The \emph{$\ell$-signature} of a vertex $v \in V(H)$ (with respect to $X$) is the set of all $\ell'$-types with $\ell' \le \ell$ that can be \emph{simulated} by $v$ in $H$. In other words, for every $\ell$-type, there exists a walk $W$ starting at $v$ such that $W = v P_0 w_0 P_1 w_1 \ldots P_\ell w_\ell P_{\ell + 1} z$ is compatible with the $\ell$-type if and only if the $\ell$-type is in the signature. We say that two vertices are \emph{$\ell$-equivalent} if their $\ell$-signatures are the same.

\begin{lemma}\label{compute-ell-signature-fpt}
One can compute in $O^*((2^{|X|}+1)^{2(\ell+2)})$ the $\ell$-signature of a vertex $v$ in $H$.
\end{lemma}

\subparagraph*{$X$-reduced sequences and equivalent journeys.}
Let $J$ be a journey and $W^X$ be the $X$-walk associated with it.
One can wonder what is really important when we consider a journey and its associated $X$-walk. Clearly, there is something special about  $X$-important waiting vertices and the conflict triples that happen before sliding to the next $X$-important waiting vertex. But what is really important in those $X$-transition walks? The only purpose of these walks (with respect to $X$) is basically to link the $i$-th $X$-important waiting vertex to the $(i+1)$-th $X$-important waiting vertex. But we cannot say that the walk is completely irrelevant since we cannot select any walk to connect these two vertices. 
Indeed, there might be some vertices of a walk whose neighborhood in $X$ actually contains a vertex on which there is a token (or there might be $H$-conflicts).
By definition of an $X$-transition walk, the neighborhood of the walk between two $X$-important waiting vertices in $X$ must be empty of tokens for the transition to happen. So (assuming no $H$-conflicts) any walk having the same $X$-trace would be ``equivalent'' to the considered walk.
In other words, if we have another walk from $w_i$ to $w_{i+1}$ which avoids the same subset of vertices in $X$ we can replace the current $X$-transition walk by it (again assuming no $H$-conflicts).

Let $J$ be a journey with exactly $r$ $X$-important waiting vertices (in its $X$-walk). Let $w_i$ and $P_i$ be respectively the $i$-th $X$-important waiting vertex and the $i$-th $X$-transition walk. Let $P_{r+1}$ be the final $X$-transition walk. Let us denote by $W_i$ the neighborhoods of $w_i$ in $X$, and by $Y_i$ the neighborhood of $P_i$ in $X$.
Let $I$ and $F$ be the neighborhoods of the initial and final vertices of the walk associated with $J$, respectively.
The \emph{type $T$ of the journey $J$} is $I (Y_i W_i)_{i \le r} Y_{r+1} F$. 
%

\begin{definition}
Two journeys are \emph{$X$-equivalent} whenever the following holds:
\begin{itemize}
\item They have the same number of $X$-important waiting vertices;
\item The initial and final vertex of the $X$-walk have the same $X$-trace; 
\item For every $i$, the $X$-trace of the $i$th $X$-important waiting vertex is the same in both journeys;  
\item For every $i$, the $X$-trace of the $i$th $X$-transition walk is the same in both journeys.
\end{itemize}
\end{definition}

We conclude this section by introducing the notion of $X$-reduced transformations. 
Let $I,J$ be two independent sets and $X$ be a subset of vertices of $G$. A slide of a token \emph{is related to $X$} if the token is moving from or to a vertex in $X$ (possibly from some other vertex in $X$). We call such a move an \emph{$X$-move}. 

\begin{definition}
A transformation $\mathcal{R}$ from $I$ to $J$ is \emph{$X$-reduced} if the number of $X$-moves is minimized and, among the transformations that minimize the number of $X$-moves, $\mathcal{R}$ minimizes the total number of moves. 
\end{definition}

\subparagraph*{The multi-component reduction.}
Let $H$ be a connected component of $G - X$. The $\ell$-signature of $H$ is the union of the $\ell$-signatures of the vertices in $H$. Let $\mathcal{H}$ be a subset of connected components of $G - X$. We say that $H \in \mathcal{H}$ is \emph{$\ell$-dangerous for $\mathcal{H}$} if there is a $\ell$-type in the $\ell$-signature of $H$ that appears in at most $\ell$ connected components of $\mathcal{H}$. Otherwise we say that $H$ is \emph{$\ell$-safe}. If there are no $\ell$-dangerous components, we say that $\mathcal{H}$ is $\ell$-safe. One can easily prove the following using iterated extractions:

\begin{lemma}\label{lem:safecomp}
Let $\ell = 5|X|k$. If there are more than $\ell(2^{|X|}+1)^{2(\ell+2)} + 2k + 1$ components in $G - X$, then there exists a collection of at least $2k+1$ components that are $\ell$-safe which can be found in $f(k,|X|) \cdot n^{O(1)}$-time, for some computable function $f$.
%\commentN{TODO - Explicit $f$}
\end{lemma}

We can now prove the mail result of this section:

\begin{lemma}\label{lemma-bound-conflicts}
Let $I_{s},I_{t}$ be two independent sets and $X$ be a subset of $V(G)$. Let $\mathcal{R}$ be an $X$-reduced transformation from $I_{s}$ to $I_{t}$.  Assume that there exists a subset $\mathcal{H}$ of at least $2k+1$ connected components of $G - X$ that is $(5|X|k)$-safe. Then, for every $C \in \mathcal{H}$, any journey on the component $C$ has at most $5|X|k-1$ $X$-important waiting vertices in its associated $X$-walk.
\end{lemma}
\begin{proof}[Sketch of the proof]
Assume for a contradiction that there exists a safe component $C \in \mathcal{H}$ and a journey $J$ of some token $t$ in $C$ that has at least $5|X|k$ $X$-important waiting vertices. Amongst all such journeys, select the one that reaches first its $(5|X|k)$-th $X$-important waiting vertex.
Let us denote by $I (Y_i W_i)_{i \le 5k} Y_{5k + 1}$ the type of the journey $J$ that we truncate after $Y_{5k + 1}$. And, let us denote by $v (P_i w_i)_{i \le 5k} P_{5k + 1}$ the partition of the walk into $X$-important waiting vertices and $X$-transition walks (we assume the walk starts at vertex $v \in V(C)$). 

For each $X$-important waiting vertex $w_i$, let $(q_i,x_i,t_i)$ be the important conflict associated to it.
Since there are at most $k$ labels of tokens and $|X|$ vertices in $X$, there exists a vertex $x \in X$ and a token with label $t'$ such that there exists at least $5$ waiting vertices such that the important conflict is of the form $(q,x,t')$ for some $q$. In other words, there exists $P_{i_1}, \ldots, P_{i_5}$ such that for each $P_i$ we have a triplet $(q, x, t')$ (recall that $q$ denotes the step in the reconfiguration sequence). Let us denote by $s_1,\ldots,s_5$ the steps of those  conflicts whose token label is $t'$ and whose vertex in $X$ is $x$ and such that these conflicts are important conflict triples in five different $X$-transition walks. 

The rest of the proof consists in proving that, rather than making the initial transformation, we can project $t'$ on an appropriately chosen component $C'$ of $\mathcal{H}$ distinct from $C$ and mimic the journey of $t$ between steps $s_1$ and $s_5$. In other words, $t'$ can simply follow a journey on $C'$ of the same type as that of $t$ between $s_1$ and $s_5$ and we can then safely project it back on $x$ at step $s_5$ without creating any $X$-conflicts. This implies that we can strictly reduce the number of $X$-conflicts, a contradiction to the assumption that the transformation is $X$-reduced. We then prove that we can also manage the $H$-conflicts by minimality of the journey.
\end{proof}

\begin{lemma}\label{lem:reducecomp}
Let $I_{s},I_{t}$ be two independent sets and $X$ be a subset of $V(G)$. If $G - X$ contains at least $4k + 2$ $(5|X|k)$-safe components, then we can delete one of those components, say $C$, such that there is a transformation from $I_{s}$ to $I_{t}$ in $G$ if and only if there is a transformation in $G - V(C)$. 
\end{lemma}

\begin{proof}[Sketch of the proof]
The proof consists in proving that, since all the journeys have at most $5|X|k-1$ $X$-important waiting vertices by  Lemma~\ref{lemma-bound-conflicts}, one can easily replace a journey in a safe component by a journey in another component either by not creating any conflicts or by creating some conflicts on shorter ``time periods'' which ensures the convergence of the procedure.
\end{proof}

Combining all the results of the section, one can prove the following: 

\begin{corollary}\label{cor-bounded-bag-degree}
Given a cutset $X$, we can assume that $G - X$ has at most $5|X|k(2^{|X|}+1)^{2(5|X|k+2)} + 4k + 2 = 2^{O(|X|^2k)}$ connected components. Moreover, when the number of components is larger we can find a component to delete in  $f(k,|X|) \cdot n^{O(1)}$-time, for some computable function $f$. 
\end{corollary}


==> Short/planar_short.tex <==
\section{Planar graphs}\label{sec-planar}
This section is dedicated to showing that 
\textsc{Token sliding} on planar graphs is fixed parameter tractable when parameterized by $k$. 
The proof also relies on the reduction rules designed for the \textsc{Galactic Token Sliding} problem. We say that a galactic graph $G = (V,E)$ is planar if the underlying simple graph is planar (i.e., if the graph $G$ where all vertices are considered as planetary vertices is planar). Let $(G, k, I_s, I_t)$ be an instance of \textsc{Galactic Token Sliding} where $G$ is planar. In addition to rules R1 to R6, we design in this section a number of rules whose exhaustive application (along with rules R1 to R6) results in an equivalent instance, which we denote again by $(G, k, I_s, I_t)$, such that $G$ is planar and has maximum degree bounded by a function of $k$ (the result then follows by applying Theorem~\ref{thm:ts-bounded-degree-fpt}). We first bound the number of vertex-disjoint paths between any two vertices of $G$, and then make use of this property to bound the degree of the graph.

\subparagraph*{Many paths between pairs of vertices.}
In what follows, we always consider an arbitrary (but fixed) planar embedding of $G$. A set of vertices is \emph{empty of tokens} if it contains no vertex of $I_s \cup I_t$. A vertex of a path is \emph{internal} if it is not one of the two endpoints of the path and it is \emph{external} otherwise. A set of paths of $G$ is \emph{internally vertex disjoint} if no two paths of the set share a common internal vertex.
Let $u,v \in V(G)$ and $P, P'$ be two internally vertex-disjoint $(u,v)$-paths. Since $G$ is planar, $P \cup P'$ is a separating cycle. We denote by $G_{P, P'}$ the graph induced by $P \cup P'$ and the vertices that lie inside of $P \cup P'$. The \emph{interior} of $G_{P,P'}$ is the graph induced by the vertices of $G_{P,P'} - (P \cup P')$ and is denoted by $G^o_{P,P'}$. Let $\mathcal{P}_{P,P'}$ be a set of internally vertex-disjoint $(u,v)$-paths of $G_{P,P'}$. Two paths $P_i$ and $P_{i+1}$ in $\mathcal{P}_{P,P'}$ are \emph{consecutive} if $G_{P_i, P_{i+1}} - \{u,v\}$ is connected and if any path from an internal vertex of $P_i$ to an internal vertex of $P_{i+1}$ in $G_{P_i,P_{i+1}} - \{u,v\}$ contains no internal vertex of any other path $P_j \in \mathcal{P}_{P,P'}$ that is distinct from $P_i$ and $P_{i+1}$. Note that since $G$ is planar, a path $P \in \mathcal{P}_{P,P'}$ can be consecutive with at most two other paths of $\mathcal{P}_{P,P'}$. By a slight abuse of notation, we say that $\mathcal{P} \subseteq \mathcal{P}_{P,P'}$ is a subset of consecutive paths if there exists an ordering $P_1, \ldots, P_{|\mathcal{P}|}$ such that for every $i \leq |\mathcal{P}|-1$, $P_i$ and $P_{i+1}$ are consecutive. We denote such an ordering as a \emph{consecutive ordering}. Finally, for every $i \leq |\mathcal{P}|-1$, we refer to the graph $G_{P_i, P_{i+1}}$ as the \emph{$ith$ section} of $\mathcal{P}$ and a section is \emph{internal} if it is not the first section nor the last section of $\mathcal{P}$.

Let $u,v \in V(G)$. Note that by the multi-component reduction rule (see Section \ref{sec-components}), the number connected components of $G-\{u,v\}$ is bounded by a function of $k$. Hence we can safely assume in the remaining of this section that $G-\{u,v\}$ is connected. %(if not, we can apply the same reasoning to show that the number of vertex-disjoint $(u,v)$-path is bounded in every connected component of $G-\{u,v\}$).
Let $\mathcal{P}$ be a set of internally vertex-disjoint and consecutive $(u,v)$-paths in $G$ of size $q \geq 3$, and let $P_1, \ldots, P_q$ denote a consecutive ordering of the paths in $\mathcal{P}$. Since the paths are consecutive, there exists a path from a vertex of $P_i - \{u,v\}$ to a vertex of $P_{i+1} - \{u,v\}$ for every $i \leq q-1$. Furthermore, since $q \geq 3$, the internal vertices of such a path all belong to $G^o_{P_{i}, P_{i+1}}$. It follows that there exists a path $P_C$ from a vertex of $P_{1}-\{u,v\}$ to a vertex of $P_q-\{u,v\}$ such that every internal vertex of $P_C$ belongs to $G^o_{P_1, P_q}$. We call such a path $P_C$ a \emph{crossing path of $\mathcal{P}$}, or just a \emph{crossing path} when $\mathcal{P}$ is obvious from context. Let us note that since $G$ is planar, a vertex $v$ of $P_C$ can have neighbors in at most two sections of $\mathcal{P}$. More particularly, if $v$ belongs to $G^o_{P_i, P_{i+1}}$ for some $i$, then it cannot have neighbors in $G^o_{P_{j}, P_{j+1}}$ for any $j \neq i$. Our goal is now the following: We will show that as long as there is a "large enough" set of internally vertex-disjoint and consecutive $(u,v)$-paths $\mathcal{P}$, then we can contract an edge of a crossing path of $\mathcal{P}$. Formally, we show that the following reduction rule is safe:

\begin{itemize}
    \item Reduction rule P1: Let $u,v \in V(G)$ and let $P, P'$ be two internally vertex-disjoint $(u,v)$-paths such that $G_{P,P'} - \{u,v\}$ is empty of tokens. Let $\mathcal{P}$ be a set of internally vertex-disjoint and consecutive $(u,v)$-paths of $G_{P,P'}$ of size at least $(10k + 21)^2$. Then, there exists an edge of a crossing path of $\mathcal{P}$ contained in an internal section of $\mathcal{P}$ that can be safely contracted.
\end{itemize}

Since reduction rules R1 to R6 and P1 either delete vertices or contract edges, the graph $G$ obtained after exhaustive application of these rules is also a galactic planar graph. 

\begin{lemma}\label{lem-bounded-paths}
Let $u,v$ be two vertices of a galactic planar graph $G$ and $C$ be a connected component of $G-\{u,v\}$ on which rule $P1$ can no longer be applied. Then the number of internally vertex-disjoint $(u,v)$-paths in $C$ is at most $2k(10k+21)^3$. 
\end{lemma}

\subparagraph*{Reducing fans and combs.}
We have proved that there cannot exist too many internally vertex-disjoint paths between two vertices (by Lemma~\ref{lem-bounded-paths} combined with the multi-component reduction rule when needed). It is however not enough to bound the degree of a single vertex of a planar graph. Before proving that the degree can indeed be bounded, let us prove that we can reduce some particular substructures called fans and combs.

An \emph{$r$-fan} centered in $x$ is a graph on $r + 1$ vertices $x,x_1,\ldots,x_r$ where $x_1,\ldots,x_r$ is an induced path and $x$ is complete to $x_1,\ldots,x_r$, i.e., $x$ is adjacent to every vertex in $x_1,\ldots,x_r$. We denote by $P$ the path from $x_1$ to $x_r$ and we let $r$ be the \emph{size} of the fan. We call the \emph{interior} of an $r$-fan $I$ the set of vertices that are in the part of the plane that is enclosed by the curve $xPx$ and that does not contain the external face of the embedding. The \emph{exterior} of the fan is the set of vertices minus the interior of the fan and the vertices of the fan itself. 
We say that a fan is \emph{$I$-empty} if there is no token of the initial and target independent sets in the interior of the fan nor on the vertices of the fan itself. 
We say that a fan is \emph{$B$-empty} if there is no black hole in the interior of the fan nor on the vertices of the fan itself.
We say that an $r$-fan is \emph{safe} if no vertex but the vertices $x,x_1$ and $x_k$ have a neighbor in the exterior of the fan. We say that $x$ is \emph{$I$-complete} to the fan if $x$ is complete to all the vertices of $I$ (and to the vertices of the fan itself).
Assume that none of the previous reduction rules apply, i.e., the galactic rules and the planar rules. Then, we claim that the following reduction rule is safe:

\begin{itemize}
    \item Reduction rule P2: Let $G$ be a (galactic) graph containing a safe $r$-fan which is $I$-empty with $r \ge 3k+2$ and such that $x$ is $I$-complete to the fan. Then we can replace $I \cup \{x_2,\ldots,x_{3k+1}\}$, where $\{x_2,\ldots,x_{3k+1}\}$ denotes the induced path from $x_2$ to $x_{3k+1}$, by a path of length $3k$ whose first vertex is connected to $x_1$, the last vertex is connected to $x_{3k+2}$, and the whole path is connected to $x$.
\end{itemize}

Informally speaking, reduction rule P2 ensures that if a vertex $x$ is connected to many consecutive vertices and these vertices only have neighbors on one side of the plane (and that moreover $x$ is complete to that part of the plane), then we can replace this part by a single path. The reason this rule is safe is that we can hide as many tokens on the path, as we can initially hide tokens in the interior plus $P$. 

A case which is not handled by rule P2 is the case where the vertices of the path can now have neighbors on both sides of the plane separated by the fan. We prove that if we have a large enough such structure satisfying certain properties then we can also reduce it. We need a few additional definitions. 
An \emph{$r$-comb} is an induced path $P=x_1,\ldots,x_r$ of length $r$ plus possible pendant (degree-one) vertices on each vertex of the path where $x_2$ and $x_{r-1}$ have degree at least $3$.
A \emph{complete $r$-comb} denotes the graph consisting of an $r$-comb plus an additional vertex $x$ that is complete to the  $r$-comb.
A complete $r$-comb is \emph{one-sided} if all the edges from $x$ to $N(P)$ (which are not in the interior of the fan $x \cup V(P)$) pass through the same side of the path (the $x_1$ side or the $x_r$ side). One can easily note that every complete $r$-comb contains a one-sided complete $r$-comb of size roughly half of the initial size.

Let $C$ be a one-sided complete $r$-comb.
Let us denote by $y$ and $z$ the neighbors of respectively $x_2$ and $x_{r-1}$ that are the in the same faces of respectively $x_3$ and $x_{r-2}$. Let us denote by
$H$ the graph consisting of the edges $xy$, $xz$, $x_2y$, $x_{r-1}z$, and the path $P$. The subgraph $H$ contains two faces containing $V(P) \setminus \{ x_1,x_r \}$. Let us denote by $A$ and $B$ the regions of the plane corresponding to the interior of these faces. The \emph{interior} of the $r$-comb is the set of vertices in the regions $A$ and $B$. 
We say that the complete $r$-comb is \emph{$I$-empty} if there is no token of the initial or target independent set in the interior of the $r$-comb nor on the vertices of the comb itself nor in $N(x_2)$ nor in $N(x_{r-1})$. 
We say that the complete $r$-comb is \emph{$B$-empty} if there is no black hole in the interior of the fan nor on the vertices of the comb itself.

\begin{itemize}
    \item Reduction rule P3: Assume that $G$ contains an $I$-empty one-sided complete $r$-comb with $r \ge (3k+2)^2$. Let us denote by $p_{i_1},\ldots,p_{i_d}$ the vertices of $P$ having at least one neighbor on the $B$ side. Then, we can replace $I \cup \{p_{i_1 + 1},\ldots,p_{i_d - 1}\}$, where $\{p_{i_1 + 1},\ldots,p_{i_d - 1}\}$ denotes the induced path from $p_{i_1 + 1}$ to $p_{i_d - 1}$, by a path of length at most $3k + 1$ whose first vertex is connected to $p_{i_1}$, the last vertex is connected to $p_{i_d}$ and the whole path is connected to $x$.
\end{itemize}

We now have all the ingredients to reduce subdivided combs.
A \emph{subdivided complete $r$-comb} is a complete $r$-comb where every edge of the comb might be subdivided except the edges incident to the vertex $x$. When edges $x_ix_{i+1}$ of the path $P$ are subdivided we denote the subpath by $P_i$ and still require that the union of the paths $P_1,\ldots,P_{r-1} = P$ has to be an induced path. We call the path $P_i$ from $x_i$ to $x_{i+1}$ the \emph{$i$-th ray}. 

%\begin{remark}\label{rem:nomberneighbors}
%Assume that there does not exist more than $\ell$ internally %vertex-disjoint paths between any pair of vertices of a planar %graph $G$. Then:
%\begin{itemize}
%\item Every vertex in $G - x$ is adjacent to at most $\ell$ %rays of a subdivided comb.
%\item Every vertex in $G - x$ contains a vertex of at most %$\ell^r$ rays of a subdivided comb in its $r$-th neighborhood %(neighborhood at distance at most $r$).
%\end{itemize}
%\end{remark}

\begin{lemma}\label{lem:p-gcomb}
Let $G$ be a planar (galactic) graph and let $\ell$ be the maximum number of internally vertex-disjoint paths between any pairs of vertices of $G$. If $G$ contains a subdivided complete $r$-comb $C$, where $r \ge 18(3k+2)^2 k \cdot \ell^3$, then $G$ can be reduced.
\end{lemma}

\subparagraph{Reducing high degree vertices.}
It remains to prove that the previous reduction rules (galactic and planar) ensure that the (reduced) planar (galactic) graph has bounded degree.

\begin{lemma}\label{lem:extractcomb}
Let $T$ be a tree with $r$ prescribed vertices $X$ and maximum degree at most $\ell$. Then there exists a subdivided comb of $T$ containing at least $\lfloor \log_{\ell+1}(|X|) \rfloor$ vertices of $X$. 
\end{lemma}

\begin{lemma}
Let $G$ be a galactic planar graph. If there exists a planet vertex $v \in V(G)$ whose planetary degree is greater than $(\ell+1)^{18(3k+2)^2 k \cdot \ell^3}$ then $G$ can be reduced. 
\end{lemma}

\begin{proof}
First we note that, for every vertex $v$, we can assume that there is a bounded number of connected components attached to $v$ by Corollary~\ref{cor-bounded-bag-degree}.

Assume now that there exists a vertex $v$ that has $r$ neighbors $X$ in a component $C$ of $G - v$ and let $T$ be a Steiner tree containing all the vertices of $X$. Note that the maximum degree of $T$ is bounded by $\ell:=f(k)$; as otherwise, we have a vertex $u$ of $T$ such that there exists too many paths between $u$ and $v$ in $C$. In this case we can apply Lemma~\ref{lem-bounded-paths}. 

So $T$ contains a subdivided comb of logarithmic size by Lemma~\ref{lem:extractcomb}, i.e. a subdivided comb with at least $18(3k+2)^2 k \cdot \ell^3$ rays. And then, by Lemma~\ref{lem:p-gcomb}, the graph can be reduced.
\end{proof}

